Joint Signal Detection and Automatic Modulation Classification via Deep Learning

Signal detection and modulation classification are two crucial tasks in various wireless communication systems. Different from prior works that investigate them independently, this paper studies the joint signal detection and automatic modulation classification (AMC) by considering a realistic and complex scenario, in which multiple signals with different modulation schemes coexist at different carrier frequencies. We first generate a coexisting RADIOML dataset (CRML23) to facilitate the joint design. Different from the publicly available AMC dataset ignoring the signal detection step and containing only one signal, our synthetic dataset covers the more realistic multiple-signal coexisting scenario. Then, we present a joint framework for detection and classification (JDM) for such a multiple-signal coexisting environment, which consists of two modules for signal detection and AMC, respectively. In particular, these two modules are interconnected using a designated data structure called "proposal". Finally, we conduct extensive simulations over the newly developed dataset, which demonstrate the effectiveness of our designs. Our code and dataset are now available as open-source (https://github.com/Singingkettle/ChangShuoRadioData).

==> tables/Abbreviation.tex <==

\begin{table}[hbpt]
  \centering
  \caption{{{Summary of Abbreviations}}}
  \renewcommand\arraystretch{1.25}
  \begin{tabular}{|m{2.2cm}<{\centering}|m{4.8cm}<{\centering}|}
    \hline
    \textbf{Abbreviations} & \textbf{Notations}                                 \\
    \hline
    Adam                   & Adaptive Moment Estimation                         \\
    \hline
    ALRT                   & Average Likelihood Ratio Test                      \\
    \hline
    AMC                    & Automatic Modulation Classification                \\
    \hline
    A/P                    & Amplitude/Phase                                    \\
    \hline
    ASK                    & Amplitude-Shift Keying                             \\
    \hline
    AWGN                   & Additive White Gaussian Noise                     \\

    \hline
    BiGRU                  & Bidirectional Gated Recurrent Unit                \\


    \hline
    CLDNN                  & Convolutional Long Short-term Deep Neural Network \\
    \hline
    CNN                    & Convolutional Neural Network                      \\
    \hline
    CNN4                   & Convolutional Neural Network with four layers                     \\
    \hline
    Decision Tree          & DT                                                \\
    \hline
    DenseNet               & Densely Connected Networks                        \\
    \hline
    DSCLDNN                & Dual-Stream CLDNN                                 \\

    \hline
    FB                     & Feature-Based                                     \\
    \hline
    FLOPs                  & Floating Point Operations Per Second              \\

    \hline
    GLRT                   & Generalized Likelihood Ratio Test                 \\
    \hline
    GPU                    & Graphic Processing Unit                           \\

    \hline
    HCGDNN                 & Hierarchical Classification Head based Convolutional Gated Deep Neural Network                      \\
    \hline
    HLRT                   & Hybrid Likelihood Ratio Test                      \\

    \hline
    I/Q                    & In-phase/Quadrature                                \\

    \hline
    KNN                    & K-Nearest Neighbor                                \\


    \hline
    LA                     & Link Adaption                                   \\
    \hline
    LB                     & Likelihood-Based                                  \\
    \hline
    LSTM                   & Long Short-term Memory Network                    \\


    \hline
    MAA                    & Mean Average Accuracy                             \\
    \hline
    MAF                    & Mean Average F1 Score                             \\
    \hline
    MLDNN                  & Multi-Task Learning based Deep Neural Network     \\

    \hline
    NLP                    & Natural Language Processing                       \\

    \hline
    PDF                    & Probability Density Function                      \\
    \hline
    PSK                    & Phase-Shift Keying                                \\

    \hline
    QAM                    & Quadrature Amplitude Modulation                   \\

    \hline
    ReLU                   & Rectified Linear Unit                        \\
    \hline
    ResNet                 & Residual Networks                                 \\
    \hline
    RNN                    & Recurrent Neural Network                          \\

    \hline
    SNR                    & Signal to Noise Ratio                             \\
    \hline
    SVM                    & Supported Vector Machine                          \\
    \hline
\end{tabular}
\label{tab:tab-1}
\end{table}

==> tables/table1.tex <==
\begin{table}[hbpt]
  \centering
  \caption{{{Modulation mode prediction in different modulation modes}}}
  \renewcommand\arraystretch{1.25}
  \begin{tabular}{c c c c c c }
    \hline
    \textbf{ } & \textbf{BPSK} & \textbf{QPSK} & \textbf{8PSK} & \textbf{16QAM}  & \textbf{64QAM}  \\
    \hline
    ideal	&	0.994505	&	0.929385	&	0.906149	&	0.895735	&	0.88189 \\
    \hline										
    real	&	0.917847	&	0.62963	&	0.588859	&	0.562963	&	0.332046 \\
    \hline		
\end{tabular}
\label{tab:table1}
\end{table}
